Trainability issues in quantum policy gradients

This research explores the trainability of Parameterized Quantum circuit-based policies in Reinforcement Learning, an area that has recently seen a surge in empirical exploration. While some studies suggest improved sample complexity using quantum gradient estimation, the efficient trainability of these policies remains an open question. Our findings reveal significant challenges, including standard Barren Plateaus with exponentially small gradients and gradient explosion. These phenomena depend on the type of basis-state partitioning and mapping these partitions onto actions. For a polynomial number of actions, a trainable window can be ensured with a polynomial number of measurements if a contiguous-like partitioning of basis-states is employed. These results are empirically validated in a multi-armed bandit environment.

==> tex_files/qpg_alleviating_variance_lemmas.tex <==
\section{Alleviating BPs in Born policies}\label{sec: alleviating BPs Born}
    This section propose strategies to alleviate the cost-function dependent BP using Born policies. In a first instance, the trivial scenario of product states is analyzed further proposed for arbitrary states.
    %\subsection{The instructive case of product states}\label{subsec: product states}
    In \cite{cerezo_cost_2021} the authors considered a simple toy model composed of an Rx-parameterized circuit. That is, for a $n$-qubit system, the parameterized unitary $V(\theta) = \bigotimes_{i=0}^{n-1} e^{-i \theta_i \sigma_x}$ was considered. The authors considered the global observable $O_G = 1 - |0\rangle \langle 0|$ with the goal of preparing the all-zero state. Even though such PQC correspond to a single layer of parameterized Pauli rotations forming a separable state, the authors showed that it already suffered from BPs. Moreover, the authors proved that since the global observable produces the cost function $C_G = 1 - \prod_{i=0}^{n-1}cos(\theta)^2$ composed of a product of cosines, the variance of cost function decays exponentially with the number of qubits and the cause is in fact the globality of the observable. The authors then suggested the local observable composed by individual qubit contributions $O_L = 1 - \sum_{j=0}^{n-1}\ket{0}\bra{0}_j \otimes \mathbb{I}_{\bar{j}}$ with local cost function $C_G = 1 - \frac{1}{n}\sum_{i=0}^{n-1}cos(\theta)^2$. Following this cost function, the authors showed that the variance of the cost function decays polynomially with the number of qubits rather then exponentially, thus avoiding BPs. This result highlights the importance of a well crafted cost-function. 

    In the context of machine learning in general, cost-functions such as the \textit{log-likelihood} often consider the score function $\log |0\rangle \langle 0|$ , instead of directly the probability as considered in the above example. Such cost-function incur a different behavior. Recall that the toy example considered before represents a separable state and thus the probability associated to the global projector $O_G = |0\rangle \langle 0|$ is equivalent to the probability obtained from the product of individual qubit contributions. That is, for an arbitrary product state $|\psi\rangle$, the probability of the all-zero state is given as
    \begin{equation}
        |\braket{0}{\psi}|^2 = \prod_{i=0}^{n-1} |\braket{0_i}{\psi}|^2
    \end{equation}
    The product of individual qubit contributions is a key property for every product state. Such property allows, and is sufficient, to prove that arbitary product states do not suffer from BPs once the score function is desired.
    The above result concerns to the log-likelihood cost function and can be applied to quantum generative learning, since the policy works the same way of Born machines \cite{benedetti_generative_2019,gili_evaluating_2022}. Nonetheless, the same reasoning can be applied the REINFORCE cost function considered in the context of RL, since the core of the objective function concerns with the log policy gradient which can be viewed as the log-likelihood once more. In that regard, the Born policy with trivial partition $|A|=2^n$ with global projector associated to action $a$ , $\ket{a}\bra{a}$ can be represented as the standard Born measurement $\pi(a|s,\theta) = |\braket{a}{\psi(s,\theta)}|^2$. However, since the parameterized state corresponds to a product state, the Born probability can be decomposed by the product of individual qubit contributions such as 

    \begin{equation}
        \pi(a|s,\theta) = |\braket{a}{\psi(s,\theta)}|^2 = \prod_{i=0}^{n-1} |\braket{a_i}{\psi(s,\theta)}|^2
        \label{eq: born policy product state decomposition}
    \end{equation}
    where $a_i$ indicates the individual qubit projector $\ket{a_i}\bra{a_i} \otimes \mathbb{I}_{\hat{i}}$ on the $i^{\text{th}}$ qubit and applying the identity operation on the remaining qubits.
    \begin{restatable}{lem}{bornproductstates}
        \label{lemma: local born pg variance}
        Consider a $n$-qubit Born policy $\pi(a|s,\theta)$ as in Definition \ref{def: born policy} with $|A|=2^n$ acting on a \textit{product state}. The probability of measuring a basis state $\ket{a}$ is given the product $\prod_{i=0}^{n-1} |\langle a_i | \psi(s,\theta)\rangle|^2 $. Then, the policy gradient variance is lower bounded by
        
        \begin{equation}
        \mathbb{V}_{\theta}\biggl[\nabla_{\theta} v_{\pi}(s) \biggr] \in \Omega \biggl(\frac{R_{max}^2 T^4 n }{(1-\gamma)^4}\biggr)
        \end{equation}
    \end{restatable}
    Lemma \ref{lemma: local born pg variance} indicates a lower bound for the variance of such cost function in terms of relevant quantities used in RL, same as considered in the Lemmas \ref{lemma: softmax pg variance} and \ref{lemma: born pg variance}. It indicates that the variance actually increases with the number of qubits. The proof for the lower bound is based on Corollary 2 from \cite{cerezo_cost_2021}, restated below as Corollary \ref{corollary: cerezo lower bound} for completion.
    
    \begin{restatable}{corollary}{cerezolowerbound}
        \label{corollary: cerezo lower bound}
        Let $C(\theta) = Tr[O \rho]$ be a cost function and $O$ an $m$-local operator where each $\widehat{O}_i$ acts non-trivially on at most $m$ qubits expressed as $\widehat{O}_i=\widehat{O}_i^{\mu_i} \otimes \widehat{O}_i^{\mu_i^{\prime}}$ $O=c_0 \mathbb{I}+\sum_{i=1}^N c_i \widehat{O}_i^{\mu_i} \otimes \widehat{O}_i^{\mu_i^{\prime}}$ where $\widehat{O}_i^{\mu_i}$ are operators acting on $m / 2$ qubits. If one term $c_i^2 \epsilon\left(\rho_{k, k^{\prime}}\right) \epsilon\left(\widehat{O}_i\right)$ vanishes no faster than $\Omega(1 / \operatorname{poly}(n))$, and if the number of layers $L$ is $\mathcal{O}(\log (n))$, then
    $$
    \mathbb{V}_{\theta} \bigl[ C(\theta) \bigr] \in \Omega\left(\frac{1}{\operatorname{poly}(n)}\right) .
    $$
    On the other hand, if at least one term $c_i^2 \epsilon\left(\rho_{k, k^{\prime}}\right) \epsilon\left(\widehat{O}_i\right)$ vanishes no faster than $\Omega\left(1 / 2^{\operatorname{poly}(\log (n))}\right)$, and if the number of layers is $\mathcal{O}(\operatorname{poly}(\log (n)))$, then
    $$
    \mathbb{V}_{\theta} \bigl[ C(\theta) \bigr] \in \Omega\left(\frac{1}{2^{\operatorname{poly}(\log (n))}}\right) .
    $$
    If $L \in \mathcal{O}(\operatorname{\operatorname{poly}}(\log (n)))$ the lower bound vanishes between polynomially and exponentially.
    \end{restatable}
    where $\epsilon(M) = D_{\text{HS}}(M,\text{Tr}[M]\frac{\mathbb{I}}{d_M}) = \text{Tr}[(M - \text{Tr}[M]\frac{\mathbb{I}}{d_M})^2]$ is the Hilbert-schmidt distance between operator $M$ and the maximally mixed state of dimension $d_M$, the dimension of $M$. In addition, $\rho_{k,k'}$ is the partial \text{Tr}ace of the input state $\rho$ down to the subsystems $S_k S_{k+1} \dots S_{k'}$. This corollary has a deep implication on both the employed observable as well the input quantum state. Both the observable and the reduced density matrices of the input for any set adjacent qubits in the light-cone need to be far (in Hilbert-Schmidt distance) from the identity matrix \cite{leone_practical_2022}, otherwise the variance will be exponentially vanishing. In the case of Born policies applied to product states, it is possible to express the observable in terms of single qubit projectors, and it can be easily verified that the Hilbert-Schmidt distance $D_{\text{HS}}(P_v,\text{Tr}[P_v]\frac{\mathbb{I}}{d_{P_v}})=\frac{1}{2}$. The multiplicative factor $c=1$ in this case. The complete proof is presented in Appendix \ref{appendix: born product states}. \\
    \begin{figure}[!htb]
        \centering
        \begin{minipage}[t]{\textwidth}
        \centering
        \includegraphics[height=0.18\textheight,width=\linewidth]{images/random circuit expectation log policy gradient.png}
        \end{minipage}%
        \hfill
        \caption[]{Expectation value of the log policy in randomly generated product states. On the left it is represented the randomly generated quantum circuit representing a product state. $P$ is sampled from $P \sim \{I, R_x, R_y, R_z\}$. On the right the expectation value of the gradient of cost functions as a function of the number of qubits and layers.}
        \label{fig: results_product_state}
    \end{figure}

    Figure \ref{fig: results_product_state} illustrates the expectation value of randomly generated product states. It can be observed the difference between the gradient norms of the standard probability cost function (prob) and the log probability or score function (log prob) as a function of the number of qubits and layers. A layer is composed of randomly sampled unitaries from the Pauli group applied to each of $n$ qubits in the tensor product Hilbert space ($\mathbb{C}^{\otimes n}$). The expectation value is empirically estimated from an average of $10^4$ randomly generated product states varying the number of qubits and layers in the range $\{2,3, \dots, 12\}$ and $\{1,2, \dots,8\}$, respectively. An asymptotically increasing expectation value with both the number of qubits and layers, can be observed, in the case of the log prob cost as opposed to the prob cost, in which the expectation value is already zero or near zero since the beginning of training. Such result serve as an empirical verification of Lemma \ref{appendix: born product states}, showcasing that the expectation value actually increases with the number of qubits and layers and is thus absent of BPs.






==> tex_files/qpg_variance_lemmas_softmax.tex <==

\begin{restatable}{lem}{softmaxpolicygradientlemma}
    \label{lemma: softmax pg variance}
    Consider a $n$-qubit softmax policy with an action's numerical preference represented by the expectation value of an observable $O_a$ constituted by the sum of $m$ global terms, as indicated in Definition \ref{def: softmax policy}. Then, if each block of a parameterized circuit forms a local 2-design, the policy gradient variance 
    \begin{equation}
        \mathbb{V}_{\theta}\biggl[\partial_{\theta} v_{\pi}(s) \biggr] \in \mathcal{O} \biggl(\frac{R_{max}^2 T^4}{(1-\gamma)^4} \frac{|A|m }{\alpha^n} \biggr)
    \end{equation}
    for $\alpha > 1$.
\end{restatable}
The proof is presented in detail in Appendix \ref{appendix: softmax pg variance}. Lemma \ref{lemma: softmax pg variance} indicates that the variance of the policy gradient increase with standard RL quantities, sames as the Born policy. Additionaly, if $O_a$ behaves globally in a PQC formed by local 2-designs parameterized blocks, then the variance of the policy gradient will decay exponentially with the number of qubits.
\noindent

\begin{restatable}{lem}{bornproductstates}
    \label{lemma: local born pg variance}
    Consider a $n$-qubit Born policy $\pi(a|s,\theta)$ as in Definition \ref{def: born policy} with $|A|=2^n$ acting on a \textit{product state}. The probability of measuring a basis state $\ket{a}$ is given the product $\prod_{i=0}^{n-1} |\langle a_i | \psi(s,\theta)\rangle|^2 $. Then, the policy gradient variance is lower bounded by
    
    \begin{equation}
    \mathbb{V}_{\theta}\biggl[\nabla_{\theta} v_{\pi}(s) \biggr] \in \Omega \biggl(\frac{R_{max}^2 T^4 n }{(1-\gamma)^4}\biggr)
    \end{equation}
\end{restatable}
Lemma \ref{lemma: local born pg variance} indicates a lower bound for the variance of such cost function in terms of relevant quantities used in RL, same as considered in the Lemmas \ref{lemma: softmax pg variance} and \ref{lemma: born pg variance}. It indicates that the variance actually increases with the number of qubits. The proof for the lower bound is based on Corollary 2 from \cite{cerezo_cost_2021}, restated below as Corollary \ref{corollary: cerezo lower bound} for completion.

\begin{restatable}{corollary}{cerezolowerbound}
    \label{corollary: cerezo lower bound}
    Let $C(\theta) = Tr[O \rho]$ be a cost function and $O$ an $m$-local operator where each $\widehat{O}_i$ acts non-trivially on at most $m$ qubits expressed as $\widehat{O}_i=\widehat{O}_i^{\mu_i} \otimes \widehat{O}_i^{\mu_i^{\prime}}$ $O=c_0 \mathbb{I}+\sum_{i=1}^N c_i \widehat{O}_i^{\mu_i} \otimes \widehat{O}_i^{\mu_i^{\prime}}$ where $\widehat{O}_i^{\mu_i}$ are operators acting on $m / 2$ qubits. If one term $c_i^2 \epsilon\left(\rho_{k, k^{\prime}}\right) \epsilon\left(\widehat{O}_i\right)$ vanishes no faster than $\Omega(1 / \operatorname{poly}(n))$, and if the number of layers $L$ is $\mathcal{O}(\log (n))$, then
$$
\mathbb{V}_{\theta} \bigl[ C(\theta) \bigr] \in \Omega\left(\frac{1}{\operatorname{poly}(n)}\right) .
$$
On the other hand, if at least one term $c_i^2 \epsilon\left(\rho_{k, k^{\prime}}\right) \epsilon\left(\widehat{O}_i\right)$ vanishes no faster than $\Omega\left(1 / 2^{\operatorname{poly}(\log (n))}\right)$, and if the number of layers is $\mathcal{O}(\operatorname{poly}(\log (n)))$, then
$$
\mathbb{V}_{\theta} \bigl[ C(\theta) \bigr] \in \Omega\left(\frac{1}{2^{\operatorname{poly}(\log (n))}}\right) .
$$
If $L \in \mathcal{O}(\operatorname{\operatorname{poly}}(\log (n)))$ the lower bound vanishes between polynomially and exponentially.
\end{restatable}
where $\epsilon(M) = D_{\text{HS}}(M,\text{Tr}[M]\frac{\mathbb{I}}{d_M}) = \text{Tr}[(M - \text{Tr}[M]\frac{\mathbb{I}}{d_M})^2]$ is the Hilbert-schmidt distance between operator $M$ and the maximally mixed state of dimension $d_M$, the dimension of $M$. In addition, $\rho_{k,k'}$ is the partial \text{Tr}ace of the input state $\rho$ down to the subsystems $S_k S_{k+1} \dots S_{k'}$. This corollary has a deep implication on both the employed observable as well the input quantum state. Both the observable and the reduced density matrices of the input for any set adjacent qubits in the light-cone need to be far (in Hilbert-Schmidt distance) from the identity matrix \cite{leone_practical_2022}, otherwise the variance will be exponentially vanishing. In the case of Born policies applied to product states, it is possible to express the observable in terms of single qubit projectors, and it can be easily verified that the Hilbert-Schmidt distance $D_{\text{HS}}(P_v,\text{Tr}[P_v]\frac{\mathbb{I}}{d_{P_v}})=\frac{1}{2}$. The multiplicative factor $c=1$ in this case. The complete proof is presented in Appendix \ref{appendix: born product states}. \\
